Affinity-aware Serverless Function Scheduling

Functions-as-a-Service (FaaS) is a Serverless Cloud paradigm where a platform manages the scheduling (e.g., resource allocation, runtime environments) of stateless functions. Recent work proposed using domain-specific languages to express per-function policies, e.g., policies that enforce the allocation on nodes that enjoy lower latencies to databases and services used by the function. Here, we focus on affinity-aware scenarios, i.e., where, for performance and functional requirements, the allocation of a function depends on the presence/absence of other functions on nodes. We present aAPP, an extension of a declarative, platform-agnostic language that captures affinity-aware scheduling at the FaaS level. We implement an aAPP-based prototype on Apache OpenWhisk. Besides proving that a FaaS platform can capture affinity awareness using aAPP and improve performance in affinity-aware scenarios, we use our prototype to show that aAPP imposes no noticeable overhead in scenarios without affinity constraints.

==> app_plus.tex <==
% !TeX root = ./main.tex
\section{The scheduling language \appp}
\label{sec:app}

% \newcommand{\DBTag}{\texttt{db\_query}}
% \newcommand{\Fname}{\texttt{big\_q}}
% \newcommand{\DBw}{\hlopt{DB\_w1}}
% \newcommand{\DBww}{\hlopt{DB\_w2}}
% \newcommand{\notDBw}{\hlopt{notDB\_w}}

% \newcommand{\mOpt}[1]{\colorbox{gray!12}{\(#1\)}}
\begin{figure}[h]
\begin{minipage}{.73\textwidth}
\begin{adjustbox}{width=.80\textwidth}
\begin{minipage}{\textwidth}
\vspace{-1.5em}
\[
\begin{array}{lll}
&& \hspace{.12\textwidth} \textit{id} \in \textit{Identifiers} 
\hspace{.1\textwidth} n \ \in \ \mathbb{N} 
\\[.5em]
\textit{app}         & \Coloneqq & \many{- \textit{tag}}
\\
\textit{tag}         & \Coloneqq & \textit{id} \ \hlstr{:} \ \many{\mathtt{-}\ \textit{block} } \quad \mOpt{\hln{followup}\ \hlstr{:}\ \fopt}
\\
\textit{block}       & \Coloneqq & \hln{workers} \ \hlstr{:}\ \wopt
\quad \mOpt{\hln{strategy} \ \hlstr{:}\ \sopt}
\quad \mOpt{\hln{invalidate} \ \hlstr{:}\ \many{-\ \iopt}}
\\
\wopt      & \Coloneqq & \hlopt{*} \Div \many{\mathtt{-}\ \textit{id}}
\\
\sopt      & \Coloneqq & \hlopt{any} %\Div \hlopt{platform} 
              \Div \hlopt{best\_first}
\\
\iopt      & \Coloneqq & \hlopt{capacity\_used} \ n \hlopt{\%} \Div \hlopt{max\_concurrent\_invocations} \ n %\Div \hlopt{overload}
\\
\fopt      & \Coloneqq & \hlopt{default} \Div \hlopt{fail}
\end{array}
\]
\vspace{-1em}
\end{minipage}
\end{adjustbox}
\caption{\label{fig:app_syntax} \app syntax.}
\end{minipage}
\hspace{-1.2em}{\color{gray}\vrule}\hspace{0em}
\begin{minipage}{.26\textwidth}
\begin{adjustbox}{width=\textwidth}
\begin{minipage}{1.2\textwidth}
\vspace{.5em}
\begin{codeEnv}
\begin{lstlisting}[xleftmargin=-1.2em, language=yaml, mathescape, basicstyle=\linespread{1}\footnotesize\ttfamily]
- f_tag:
  - $\hln{workers}$:
      - w1
      - w2
    $\hln{strategy}\hlstr{:}\ \hlopt{best\_first}$
    $\hln{invalidate}$:
      - $\hlopt{capacity\_used}$ 80%
  $\hln{followup}\hlstr{:}\ \hlopt{fail}$
\end{lstlisting}
\end{codeEnv}
% \end{adjustbox}
\end{minipage}
\end{adjustbox}
\vspace{1.5em}
\caption{\label{fig:app_example} Example \app script.}
\end{minipage}
\vspace{-2em}
\end{figure}

The syntax of \app draws inspiration from YAML~\cite{web:YAML}, a renowned
data-serialisation language for configuration files---e.g., many modern tools
use the format, like Kubernetes, Ansible, and Docker. While \app scripts are
YAML-compliant, we slightly stylise the \app syntax to increase readability (for
instance, we omit quotes around strings, e.g., \hlopt{*} instead of
\hlopt{"*"}). For simplicity, we also assume two minor variations. First, we
cover the whole syntax of \app~\cite{PGMZ20} except for two options,
\hln{strategy}\hlstr{:} \hlopt{platform} and \hln{invalidate}\hlstr{:}
\hlopt{overload}, which we avoid modelling since they are platform-specific
(e.g., in Apache OpenWhisk \hlopt{platform} implies the usage of its hardcoded
strategy, based on a co-prime heuristic selection logic~\cite{PGMZ20}). Second,
we rename the \hlopt{random} strategy option to \hlopt{any}, to point out that
it performs non-deterministic worker selection instead of a
uniformly-distributed one, as \hlopt{random} does---the change allows us to
avoid introducing more involved quantitative semantics needed to capture probabilities, left as future work.
%
% capture e.g., a uniformly distributed selection of workers as the
% \hlopt{random} option does---although the authors do not rigorously define the
% statistics behind the \hlopt{random} strategy~\cite{PGMZ20,DGMTZ22}.

% We deem the
% exploration of quantitative semantics an important step, but we consider it
% future work and prefer to proceed with a simpler model and pave the way for more
% involved future formalisations.

We report in \cref{fig:app_syntax} the syntax of \app considered in this paper.
From here on, we indicate syntactic units in \emph{italics}, optional fragments
in \(\mOpt{grey}\), terminals in \code{monospace}, and lists with
\(\many{bars}\).

Summarising, the fundamental ingredients of \app are: \textit{i)} named
scheduling policies identified by a \textit{tag} and \textit{ii)} policy
\(\textit{block}\)s that indicate either some collection of workers, each
identified by a worker \textit{id}, or the universal \hlopt{*}. Each tag can
define a \hln{followup} clause, which specifies what to do if the policy of the
tag did not lead to the scheduling of the function; either \hlopt{fail}, to
terminate the scheduling, or \hlopt{default} to apply the special
\texttt{default}-tagged policy.
%
Each block can define a \hln{strategy} for worker selection---$\hlopt{any}$
selects non-deterministically one of the available workers in the list;
$\hlopt{best\_first}$ selects the first available worker in the list---and a
list of \hln{invalidate} constraints that invalidate a worker for the
allocation---$\hlopt{capacity\_used}$ invalidates a worker if its resource
occupation reaches the set threshold; $\hlopt{max\_concurrent\_invocations}$
invalidates a worker if it hosts more than the specified number of functions.

In \cref{fig:app_example}, we show an \app policy tagged \texttt{f\_tag}, used in the examples of this section.





==> conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

The implementation and validation of the \appp-based OpenWhisk allowed us to
effectively tackle the challenge of enforcing affinity and anti-affinity constraints in a FaaS platform.
Our approach involved enhancing the Controller component to parse \appp scripts and integrate a new scheduler 
capable of enforcing these constraints. Through experimentation using the presented use case,
we have demonstrated the effectiveness of the \appp platform in reducing latency and tail latency compared 
to scenarios without affinity constraints. These findings underscore the importance of considering affinity requirements, 
particularly in multi-zone execution contexts.

Furthermore, benchmarking tests have shown that the overhead of supporting \appp-based affinity constraints is minimal 
compared to vanilla OpenWhisk and its \app-based variant. 

In summary, \appp allows FaaS platforms to offer support for affinity constraints that enable the users to integrate 
ad-hoc optimizations in their serverless applications.
